Progressive Boosting for Class Imbalance

Pattern recognition applications often suffer from skewed data distributions between classes, which may vary during operations w.r.t. the design data. Two-class classification systems designed using skewed data tend to recognize the majority class better than the minority class of interest. Several data-level techniques have been proposed to alleviate this issue by up-sampling minority samples or under-sampling majority samples. However, some informative samples may be neglected by random under-sampling and adding synthetic positive samples through up-sampling adds to training complexity. In this paper, a new ensemble learning algorithm called Progressive Boosting (PBoost) is proposed that progressively inserts uncorrelated groups of samples into a Boosting procedure to avoid loss of information while generating a diverse pool of classifiers. Base classifiers in this ensemble are generated from one iteration to the next, using subsets from a validation set that grows gradually in size and imbalance. Consequently, PBoost is more robust to unknown and variable levels of skew in operational data, and has lower computation complexity than Boosting ensembles in literature. In PBoost, a new loss factor is proposed to avoid bias of performance towards the negative class. Using this loss factor, the weight update of samples and classifier contribution in final predictions are set based on the ability to recognize both classes. Using the proposed loss factor instead of standard accuracy can avoid biasing performance in any Boosting ensemble. The proposed approach was validated and compared using synthetic data, videos from the FIA dataset that emulates face re-identification applications, and KEEL collection of datasets. Results show that PBoost can outperform state of the art techniques in terms of both accuracy and complexity over different levels of imbalance and overlap between classes.

==> finalbbl.tex <==
\begin{thebibliography}{10}
\expandafter\ifx\csname url\endcsname\relax
  \def\url#1{\texttt{#1}}\fi
\expandafter\ifx\csname urlprefix\endcsname\relax\def\urlprefix{URL }\fi
\expandafter\ifx\csname href\endcsname\relax
  \def\href#1#2{#2} \def\path#1{#1}\fi

\bibitem{galar2011overview}
M.~Galar, A.~Fern{\'a}ndez, E.~Barrenechea, H.~Bustince, F.~Herrera, An
  overview of ensemble methods for binary classifiers in multi-class problems:
  Experimental study on one-vs-one and one-vs-all schemes, Pattern Recognition
  44~(8) (2011) 1761--1776.

\bibitem{wang2012multiclass}
S.~Wang, X.~Yao, Multiclass imbalance problems: Analysis and potential
  solutions, IEEE Transactions on Systems, Man, and Cybernetics, Part B
  (Cybernetics) 42~(4) (2012) 1119--1130.

\bibitem{he2009learning}
H.~He, E.~A. Garcia, Learning from imbalanced data, Knowledge and Data
  Engineering, IEEE Transactions on 21~(9) (2009) 1263--1284.

\bibitem{galar2012review}
M.~Galar, A.~Fernandez, E.~Barrenechea, H.~Bustince, F.~Herrera, A review on
  ensembles for the class imbalance problem: Bagging-, Boosting-, and
  hybrid-based approaches, Systems, Man, and Cybernetics, Part C: Applications
  and Reviews, IEEE Transactions on 42~(4) (2012) 463--484.

\bibitem{radtke2014skew}
P.~V. Radtke, E.~Granger, R.~Sabourin, D.~O. Gorodnichy, Skew-sensitive Boolean
  combination for adaptive ensembles--an application to face recognition in
  video surveillance, Information Fusion 20 (2014) 31--48.

\bibitem{de2015adaptive}
M.~De-la Torre, E.~Granger, R.~Sabourin, D.~O. Gorodnichy, Adaptive
  skew-sensitive ensembles for face recognition in video surveillance, Pattern
  Recognition 48~(11) (2015) 3385--3406.

\bibitem{icpram2016TUS}
R.~Soleymani, E.~Granger, G.~Fumera, Classifier ensembles with trajectory
  under-sampling for face re-identification, in: Proceedings of the
  International Conference on Pattern Recognition Applications and
  Methods-Volume 1, SCITEPRESS-Science and Technology Publications, Lda, 2016,
  pp. 97--108.

\bibitem{freund1995desicion}
Y.~Freund, R.~E. Schapire, A desicion-theoretic generalization of on-line
  learning and an application to Boosting, in: Computational learning theory,
  Springer, 1995, pp. 23--37.

\bibitem{freund1996experiments}
Y.~Freund, R.~E. Schapire, et~al., Experiments with a new Boosting algorithm,
  in: Machine Learning and Applications, 1996. ICMLA'96 International
  Conference on, 1996.

\bibitem{chawla2003smoteboost}
N.~V. Chawla, A.~Lazarevic, L.~O. Hall, K.~W. Bowyer, SMOTEBoost: Improving
  prediction of the minority class in Boosting, in: European Conference on
  Principles of Data Mining and Knowledge Discovery, Springer, 2003, pp.
  107--119.

\bibitem{hu2009msmote}
S.~Hu, Y.~Liang, L.~Ma, Y.~He, Msmote: improving classification performance
  when training data is imbalanced, in: Proceedings of the 2009 Second
  International Workshop on Computer Science and Engineering, Vol.~2, Citeseer,
  2009, pp. 13--17.

\bibitem{mease2007cost}
D.~Mease, A.~Wyner, A.~Buja, Cost-weighted Boosting with jittering and
  over/under-sampling: Jous-boost, J. Machine Learning Research 8 (2007)
  409--439.

\bibitem{guo2004learning}
H.~Guo, H.~L. Viktor, Learning from imbalanced data sets with Boosting and data
  generation: the databoost-im approach, ACM SIGKDD Explorations Newsletter
  6~(1) (2004) 30--39.

\bibitem{seiffert2010rusboost}
C.~Seiffert, T.~M. Khoshgoftaar, J.~Van~Hulse, A.~Napolitano, RusBoost: A
  hybrid approach to alleviating class imbalance, Systems, Man and Cybernetics,
  Part A: Systems and Humans, IEEE Transactions on 40~(1) (2010) 185--197.

\bibitem{galar2013eusboost}
M.~Galar, A.~Fern{\'a}ndez, E.~Barrenechea, F.~Herrera, EusBoost: Enhancing
  ensembles for highly imbalanced data-sets by evolutionary undersampling,
  Pattern Recognition 46~(12) (2013) 3460--3471.

\bibitem{diez2015random}
J.~F. D{\'\i}ez-Pastor, J.~J. Rodr{\'\i}guez, C.~Garc{\'\i}a-Osorio, L.~I.
  Kuncheva, Random Balance: Ensembles of variable priors classifiers for
  imbalanced data, Knowledge-Based Systems 85 (2015) 96--111.

\bibitem{fan1999adacost}
W.~Fan, S.~J. Stolfo, J.~Zhang, P.~K. Chan, Adacost: misclassification
  cost-sensitive Boosting, in: Machine Learning and Applications, 1999.
  ICMLA'99 International Conference on, 1999.

\bibitem{ting2000comparative}
K.~M. Ting, A comparative study of cost-sensitive Boosting algorithms, in:
  Machine Learning and Applications, 2000. International Conference on,
  Citeseer, 2000.

\bibitem{sun2007cost}
Y.~Sun, M.~S. Kamel, A.~K. Wong, Y.~Wang, Cost-sensitive Boosting for
  classification of imbalanced data, Pattern Recognition 40~(12) (2007)
  3358--3378.

\bibitem{joshi2001evaluating}
M.~V. Joshi, V.~Kumar, R.~C. Agarwal, Evaluating Boosting algorithms to
  classify rare classes: Comparison and improvements, in: Data Mining, 2001.
  ICDM 2001, Proceedings IEEE International Conference on, IEEE, 2001, pp.
  257--264.

\bibitem{kim2015geometric}
M.-J. Kim, D.-K. Kang, H.~B. Kim, Geometric mean based Boosting algorithm with
  over-sampling to resolve data imbalance problem for bankruptcy prediction,
  Expert Systems with Applications 42~(3) (2015) 1074--1082.

\bibitem{rokach2010ensemble}
L.~Rokach, Ensemble-based classifiers, Artificial Intelligence Review 33~(1-2)
  (2010) 1--39.

\bibitem{garcia2009evolutionary}
S.~Garc{\'\i}a, F.~Herrera, Evolutionary undersampling for classification with
  imbalanced datasets: Proposals and taxonomy, Evolutionary computation 17~(3)
  (2009) 275--306.

\bibitem{yan2003predicting}
R.~Yan, Y.~Liu, R.~Jin, A.~Hauptmann, On predicting rare classes with SVM
  ensembles in scene classification, in: Acoustics, Speech, and Signal
  Processing, 2003. Proceedings.(ICASSP'03). 2003 IEEE International Conference
  on, Vol.~3, IEEE, 2003, pp. III--21.

\bibitem{li2013constructing}
Q.~Li, B.~Yang, Y.~Li, N.~Deng, L.~Jing, Constructing support vector machine
  ensemble with segmentation for imbalanced datasets, Neural Computing and
  Applications 22~(1) (2013) 249--256.

\bibitem{fawcett2006introduction}
T.~Fawcett, An introduction to ROC analysis, Pattern recognition letters 27~(8)
  (2006) 861--874.

\bibitem{garcia2010theoretical}
V.~Garc{\i}a, R.~Mollineda, J.~S{\'a}nchez, Theoretical analysis of a
  performance measure for imbalanced data, in: Proceedings of the 20th
  International Conference on Pattern Recognition (ICPR’10), 2010, pp.
  617--620.

\bibitem{hernandez2012unified}
J.~Hern{\'a}ndez-Orallo, P.~Flach, C.~Ferri, A unified view of performance
  metrics: translating threshold choice into expected classification loss,
  Journal of Machine Learning Research 13~(Oct) (2012) 2813--2869.

\bibitem{flach2015precision}
P.~Flach, M.~Kull, Precision-Recall-Gain curves: PR analysis done right, in:
  Advances in Neural Information Processing Systems, 2015, pp. 838--846.

\bibitem{xu2005survey}
R.~Xu, D.~Wunsch, Survey of clustering algorithms, IEEE Transactions on neural
  networks 16~(3) (2005) 645--678.

\bibitem{goh2005cmu}
R.~Goh, L.~Liu, X.~Liu, T.~Chen, The CMU face in action (FIA) database, in:
  Analysis and Modelling of Faces and Gestures, 2005, pp. 255--263.

\bibitem{alcala2010keel}
J.~Alcal{\'a}, A.~Fern{\'a}ndez, J.~Luengo, J.~Derrac, S.~Garc{\'\i}a,
  L.~S{\'a}nchez, F.~Herrera, Keel data-mining software tool: Data set
  repository, integration of algorithms and experimental analysis framework,
  Journal of Multiple-Valued Logic and Soft Computing 17~(2-3) (2010) 255--287.

\bibitem{de2015partially}
M.~De-la Torre, E.~Granger, P.~V. Radtke, R.~Sabourin, D.~O. Gorodnichy,
  Partially-supervised learning from facial trajectories for face recognition
  in video surveillance, Information Fusion 24 (2015) 31--53.

\bibitem{pagano2014adaptive}
C.~Pagano, E.~Granger, R.~Sabourin, G.~L. Marcialis, F.~Roli, Adaptive
  ensembles for face recognition in changing video surveillance environments,
  Information Sciences 286 (2014) 75--101.

\bibitem{viola2001rapid}
P.~Viola, M.~Jones, Rapid object detection using a boosted cascade of simple
  features, in: Computer Vision and Pattern Recognition, 2001. CVPR 2001.
  Proceedings of the 2001 IEEE Computer Society Conference on, Vol.~1, IEEE,
  2001, pp. I--511.

\bibitem{ojala2002multiresolution}
T.~Ojala, M.~Pietikainen, T.~Maenpaa, Multiresolution gray-scale and rotation
  invariant texture classification with local binary patterns, Pattern Analysis
  and Machine Intelligence, IEEE Transactions on 24~(7) (2002) 971--987.

\bibitem{lopez2013insight}
V.~L{\'o}pez, A.~Fern{\'a}ndez, S.~Garc{\'\i}a, V.~Palade, F.~Herrera, An
  insight into classification with imbalanced data: Empirical results and
  current trends on using data intrinsic characteristics, Information Sciences
  250 (2013) 113--141.

\bibitem{chang2011libsvm}
C.-C. Chang, C.-J. Lin, LibSVM: a library for support vector machines, ACM
  Transactions on Intelligent Systems and Technology (TIST) 2~(3) (2011) 27.

\bibitem{li2008adaboost}
X.~Li, L.~Wang, E.~Sung, AdaBoost with SVM-based component classifiers,
  Engineering Applications of Artificial Intelligence 21~(5) (2008) 785--795.

\bibitem{dunn1973fuzzy}
J.~C. Dunn, A fuzzy relative of the isodata process and its use in detecting
  compact well-separated clusters.

\bibitem{lipton2014optimal}
Z.~C. Lipton, C.~Elkan, B.~Naryanaswamy, Optimal thresholding of classifiers to
  maximize F1 measure, in: Joint European Conference on Machine Learning and
  Knowledge Discovery in Databases, Springer, 2014, pp. 225--239.

\end{thebibliography}

